Improving Interpretability and Accuracy in Neuro-Symbolic Rule Extraction Using Class-Specific Sparse Filters

There has been significant focus on creating neuro-symbolic models for interpretable image classification using Convolutional Neural Networks (CNNs). These methods aim to replace the CNN with a neuro-symbolic model consisting of the CNN, which is used as a feature extractor, and an interpretable rule-set extracted from the CNN itself. While these approaches provide interpretability through the extracted rule-set, they often compromise accuracy compared to the original CNN model. In this paper, we identify the root cause of this accuracy loss as the post-training binarization of filter activations to extract the rule-set. To address this, we propose a novel sparsity loss function that enables class-specific filter binarization during CNN training, thus minimizing information loss when extracting the rule-set. We evaluate several training strategies with our novel sparsity loss, analyzing their effectiveness and providing guidance on their appropriate use. Notably, we set a new benchmark, achieving a 9% improvement in accuracy and a 53% reduction in rule-set size on average, compared to the previous SOTA, while coming within 3% of the original CNN's accuracy. This highlights the significant potential of interpretable neuro-symbolic models as viable alternatives to black-box CNNs.

==> related.tex <==
\section{Related Work}

% \subsection{Knowledge Extraction from Neural Networks}
Extracting knowledge from neural networks is a well studied topic \cite{ANDREWS1995373,tickle1998truth} but only recently extracting rules from CNNs by binarizing the filter outputs has gained popularity \cite{eric,eric2,nesyfold}. However, none of these approaches facilitate binarization of filter outputs like our method. Our approach addresses the performance gap between the NeSy model and the trained CNN.

% \subsection{Visualization of CNN Layers}
Previous research has primarily focused on visualizing the outputs of CNN layers, aiming to establish relationships between input pixels and neuron outputs. Zeiler et al.~\cite{zeiler2014visualizing} employ output activations as a regularizer to identify discriminative image regions. Other studies~\cite{https://doi.org/10.48550/arxiv.1412.6815,selvaraju2017grad,https://doi.org/10.48550/arxiv.1312.6034}, utilize gradients to perform input-output mapping. Unlike these visualization methods, our approach generates a logical rule set. Additionally, Ferreira et al.~\cite{KR2022-45} implement multiple mapping networks trained to link activation values from the primary network’s output to human-defined concepts within an induced logic-based theory. However, their method requires multiple auxiliary neural networks in addition to the main model.

% \subsection{CNN Explanation}
Bologna et al.~\cite{bologna2020two} extract propositional rules from CNN at the neuron level while our approach generates rule set at CNN filter level. Qi et al.~\cite{Qi2021-QIEDN} maps a high-dimensional embedding to a low-dimensional explanation space to explain predictions. Chen et al.~\cite{chen2019looks} introduce a prototype layer within the network, enabling comparisons between image parts and learned prototypes to align with how the network reasons about new examples. Zhang et al.~\cite{zhang2018interpreting,zhang2017growing} represent learned CNN concepts using a hierarchical graph while another work ~\cite{zhang2017qaforxcnn} uses active question-answering to extract latent patterns from a pre-trained CNN, constructing an interpretable And-Or graph to associate these patterns with target parts. In contrast, our work focuses on generating logical explanations based on concepts represented by CNN filters.

% % \subsection{Neuro-Symbolic Systems}
% Sen et al.~\cite{nesyilp} propose learning rules with the logical neural networks. Shindo et al. and Evans et al.~\cite{diffilpext,diffilp} induce logic rules from data using an efficient clause search method for a differentiable Inductive Logic Programming solver. 
% These systems belongs to the Neuro:Symbolic \rightarrow Neuro category whereas ours belongs to the Neuro; Symbolic category.
